Discovery of Latent Factors in High-dimensional Data Using Tensor Methods

Unsupervised learning aims at the discovery of hidden structure that drives the observations in the real world. It is essential for success in modern machine learning. Latent variable models are versatile in unsupervised learning and have applications in almost every domain. Training latent variable models is challenging due to the non-convexity of the likelihood objective. An alternative method is based on the spectral decomposition of low order moment tensors. This versatile framework is guaranteed to estimate the correct model consistently. My thesis spans both theoretical analysis of tensor decomposition framework and practical implementation of various applications. This thesis presents theoretical results on convergence to globally optimal solution of tensor decomposition using the stochastic gradient descent, despite non-convexity of the objective. This is the first work that gives global convergence guarantees for the stochastic gradient descent on non-convex functions with exponentially many local minima and saddle points. This thesis also presents large-scale deployment of spectral methods carried out on various platforms. Dimensionality reduction techniques such as random projection are incorporated for a highly parallel and scalable tensor decomposition algorithm. We obtain a gain in both accuracies and in running times by several orders of magnitude compared to the state-of-art variational methods. To solve real world problems, more advanced models and learning algorithms are proposed. This thesis discusses generalization of LDA model to mixed membership stochastic block model for learning user communities in social network, convolutional dictionary model for learning word-sequence embeddings, hierarchical tensor decomposition and latent tree structure model for learning disease hierarchy, and spatial point process mixture model for detecting cell types in neuroscience.

==> figure_cartoon.tex <==
\begin{figure}[t]
%\subfloat%[a][Convolutional sparse coding model]
{\begin{minipage}{0.6\textwidth}
\bc
\bp
\psfrag{=}[Bc]{$=$}
\psfrag{*}[Bl]{$*$}
\psfrag{X}[Tc]{$x$}
\psfrag{sum}[Cl]{ $\sum$}
\psfrag{f1}[Tl]{$f_1^*$}
\psfrag{w1}[Tl]{$w_1^*$}
\psfrag{f2}[Tl]{$f_2^*$}
\psfrag{w2}[Tl]{$w_2^*$}
\psfrag{circf}[Tc]{$\quad \mathcal{F}^*$}
\psfrag{w}[Tl]{$w^*$}
\psfrag{(a)}[Bl]{\scriptsize{\bf(a)}Convolutional model}
\psfrag{(b)}[Bl]{\scriptsize{\bf(b)}Reformulated model}
\includegraphics[width=\textwidth,height=0.8in]{\fighomeConv/1dconv-2filters.eps}
\ep
\ec
\end{minipage}
}   \hfil\setcounter{subfigure}{2}\subfloat[\scriptsize{(c)}][\scriptsize Convolutional tensor decomposition]{\begin{minipage}{0.4\textwidth}

\vspace{-0.9em}

\bc
\bp
\psfrag{=}[Bc]{\scriptsize $=$}
\psfrag{+}[Bc]{\scriptsize $+ $}
\psfrag{..}[Bc]{{\scriptsize  $\ldots$}}
\psfrag{..}[Bc]{{\scriptsize  $\ldots$}}
\psfrag{....}[Bc]{{\scriptsize  $\ldots$}}
\psfrag{M3}[Tl]{\scriptsize $\Cum$}
\psfrag{f1}[Tl]{\scriptsize $f_1^*$}
\psfrag{f2}[Tl]{\scriptsize $f_2^*$}
\psfrag{sf1}[Tc]{\scriptsize $\shift({f_1^*})$}
\psfrag{sf2}[Tc]{\scriptsize $\shift({f_2^*})$}
\psfrag{lambda1}[l]{\scriptsize $\lambda_1 (\mathcal{F}_1^*)^{\otimes 3}$}
\psfrag{lambda2}[l]{\scriptsize $\lambda_2 (\mathcal{F}_2^*)^{\otimes 3}$}
\psfrag{lambda3}[l]{\scriptsize  $ \  \ldots$}
\psfrag{lambda4}[l]{ }
\fbox{
\includegraphics[width=\textwidth,height=0.6in]{\fighomeConv/tensor-decomp-conv.eps}}
\ep
\ec\end{minipage}}
\caption[Convolutional tensor decomposition for learning convolutional ICA models]{Convolutional tensor decomposition for learning convolutional ICA models.(a) The convolutional generative model with 2 filters. (b) Reformulated model where $\CCir^*$ is column-stacked circulant matrix. (c) The third order cumulant is decomposed as filters. }
\end{figure}



%\begin{figure}[!htb]
%\subfloat%[a][Convolutional sparse coding model]
%
%\bc
%\bp
%\psfrag{=}[Bc]{\scriptsize $=$}
%\psfrag{*}[Bl]{\scriptsize $*$}
%\psfrag{X}[Bc]{\scriptsize $x$}
%\psfrag{sum}[Cl]{\scriptsize  $\sum$}
%\psfrag{fi}[Bl]{\scriptsize $f_i^*$}
%\psfrag{wi}[Bl]{\scriptsize $w_i^*$}
%\psfrag{circf}[Bc]{\scriptsize $\quad \mathcal{F}^*$}
%\psfrag{w}[Bl]{\scriptsize $w^*$}
%\psfrag{(a)}[Bl]{\scriptsize {\bf(a)}Convolutional model}
%\psfrag{(b)}[Bl]{\scriptsize {\bf(b)}Reformulated model}
%\includegraphics[width=0.5\textwidth]{1dconv-2filters.eps}
%\ep
%\ec
%%\setcounter{subfigure}{2}
%\caption{Convolutional tensor decomposition for learning convolutional ICA models.(a) The convolutional generative model with 2 filters. (b) Reformulated model where $\CCir^*$ is column-stacked circulant matrix. }
%\end{figure}
%
%
%\begin{figure}
%%\subfloat[(c)][Convolutional tensor decomposition]{\begin{minipage}{2.8in}
%\bc
%\bp
%\psfrag{=}[Bc]{\scriptsize $=$}
%\psfrag{+}[Bc]{\scriptsize $+ $}
%\psfrag{..}[Bc]{{\scriptsize  $\ldots$}}
%\psfrag{..}[Bc]{{\scriptsize  $\ldots$}}
%\psfrag{....}[Bc]{{\scriptsize  $\ldots$}}
%\psfrag{Tensor M3}[l]{\scriptsize $\Cum$}
%\psfrag{lambda1}[l]{\scriptsize $\lambda_1 (\mathcal{F}_1^*)^{\otimes 3}$}
%\psfrag{lambda2}[l]{\scriptsize $\lambda_2 (\mathcal{F}_2^*)^{\otimes 3}$}
%\psfrag{lambda3}[l]{\scriptsize  $ \  \ldots$}
%\psfrag{lambda4}[l]{ }
%\includegraphics[width=0.5\textwidth]{tensor-decomp-conv.eps}
%\ep
%\ec%\end{minipage}}
%\caption{Convolutional tensor decomposition for learning convolutional ICA models.  The CP decomposition of third order cumulant corresponds to filters and their circulant shifts. }
%\end{figure}


==> figure_compareVoxel.tex <==
\begin{figure}[ht]
\begin{center}
\psfrag{Spatial Point Process Mixture ISH Data}[Bl]{\tiny{Spatial point process (ours)}}
\psfrag{Voxel Data}[Bl]{\tiny{Average expression level (baseline)}}
\psfrag{Spatial Point Process Mixture ISH Data (Permute)}[Bl]{\tiny{Spatial point process (ours, permuted)}}
\psfrag{Voxel Data (Permute)}[Bl]{\tiny{Average expression level (baseline, permuted)}}
\psfrag{Perplexity Score}[Bl]{\tiny{Perplexity Score}}
\psfrag{Number of Hidden Cell Types}[Bl]{\tiny{Number of Cell Types}}
\includegraphics[width=3in]{\fighomeBrain/ErrorBar_NNMF_ISHSpatial_Voxel_Science_PermuteScience.eps}
%\label{fig:science_ish}
%\label{fig:permutescience_ish}\\
\caption[Comparison of gene expression profiles recovered for cell-types in the somatosensory cortex]{Comparison of gene expression profiles recovered for cell-types in the somatosensory cortex by fitting an LDA model using spatial point process features (ours) vs the standard average gene expression level feature (baseline). Our features provide a significantly better match, with lower perplexity, to ground truth single-cell RNA sequencing derived transcriptomes.  A permutation test is done to access statistical significance. Perplexity is computed by matching to surrogate single-cell RNA transcriptomes by shuffling the gene expression levels between cells. Comparing with permute test shows that our cell-types are significantly different from chance.  }
\label{fig:science}
\end{center}
\end{figure}
\vspace{-2em}
%\begin{figure}[ht]
%\subfloat[a][Perplexity evaluated on single cell RNA-seq]
%{\begin{minipage}{2.6in}\bc  
%\psfrag{Spatial Point Process Mixture ISH Data}[Bl]{\tiny{Spatial point process (ours)}}
%\psfrag{Voxel Data}[Bl]{\tiny{Average expression level (baseline)}}
%\psfrag{Perplexity Score}[Bl]{\tiny{Perplexity Score}}
%\psfrag{Number of Hidden Cell Types}[Bl]{\tiny{Number of Cell Types}}
%\includegraphics[width=2.6in]{\fighomeBrain/ErrorBar_NNMF_ISHSpatial_Voxel_Science.eps}\label{fig:science_ish}\ec\end{minipage}}\hfil
%\subfloat[b][Perplexity evaluated on permuted single cell RNA-seq]
%{\begin{minipage}{3in}\bc  
%\psfrag{Spatial Point Process Mixture ISH Data}{\tiny{Spatial point process (ours)}}
%\psfrag{Voxel Data}{\tiny{Average expression level (baseline)}}
%\psfrag{Perplexity Score}[Bl]{\tiny{Perplexity Score}}
%\psfrag{Number of Hidden Cell Types}[Bl]{\tiny{Number of Cell Types}}
%\includegraphics[width=2.6in]{\fighomeBrain/ErrorBar_NNMF_ISHSpatial_Voxel_PermuteScience.eps}
%\label{fig:permutescience_ish}\ec\end{minipage}}\\
%%\subfloat[c][Perplexity Diff: Single Cell RNA-seq vs Permuted]
%%{\begin{minipage}{3in}\bc  \psfrag{Spatial Point Process Mixture ISH Data}{\tiny{Spatial Point Process}}\psfrag{Voxel Data}{\tiny{Voxel}}\includegraphics[width=2.8in]{\fighomeBrain/ErrorBar_NNMF_ISHSpatial_Voxel_Diff.eps}\ec\end{minipage}}\\
%\caption{Comparison of gene expression profiles recovered for cell-types in the somatosensory cortex by fitting an LDA model using spatial point process features (ours) vs the standard average gene expression level feature (baseline). (a) Our features provide a significantly better match, with lower perplexity, to ground truth single-cell RNA sequencing derived transcriptomes. (b) A permutation test to access statistical significance. Perplexity is computed by matching to surrogate single-cell RNA transcriptomes by shuffling the gene expression levels between cells. Comparing (a) to (b) shows that our cell-types are significantly different from chance. Note the difference in y-axis between the two plots. }
%\label{fig:science}
%\end{figure}
